On the Utility Recovery Incapability of Neural Net-based Differential Private Tabular Training Data Synthesizer under Privacy Deregulation

Devising procedures for auditing generative model privacy-utility tradeoff is an important yet unresolved problem in practice. Existing works concentrates on investigating the privacy constraint side effect in terms of utility degradation of the train on synthetic, test on real paradigm of synthetic data training. We push such understanding on privacy-utility tradeoff to next level by observing the privacy deregulation side effect on synthetic training data utility. Surprisingly, we discover the Utility Recovery Incapability of DP-CTGAN and PATE-CTGAN under privacy deregulation, raising concerns on their practical applications. The main message is Privacy Deregulation does NOT always imply Utility Recovery.

==> z99_WriteUpDraft.tex <==



We take the privacy deregulation lens to address the privacy-utility tradeoff of synthetic data. 
Traditional privacy-utility tradeoff in fact is the privacy-general utility tradeoff, which address how privacy has effect on the distance between real and synthetic dataset. Our approach is the privacy-specific utility tradeoff, which address how privacy has effect on the performance of down-stream machine learning task. 

Current state of the community doesn't have a good framework to link the general utility to specific utility.

We provide a systematic investigation on the Utility Recovery Incapability across different family of generative models. 

Unfortunately, based on our investigation, \textbf{the Utility Recovery Incapability is universal}, across machine learning models or the real datasets.

Our framework examine 4 tabular dataset, 6 basic machine learning classification models and 3 family of generative models. 

We take the observation from two perspective

(a) Fix a single dataset, the Utility Recovery Incapability phenomenon is universal across 6 family of basic machine learning algorithms.


(b) Fix a machine learning algorithms, the Utility Recovery Incapability phenomenon is universal across 4 basic tabular datasets. 



(c) Unexpected : Sometimes, DS loose. But most time in our experiment, DS win.


\textcolor{red}{Maybe a table to summary the comparison}



\clearpage


\textbf{Paper Organization}



\textbf{Idea 4: Utility Recovery Incapability disclosure of certain family of Synthesizer.}

\textbf{Idea 5: Message, not all way to guarantee Differential Privacy are equal in terms of Specific Utility.}



---
Deregulation is the process of making a trade, business activity, etc. free from rules and controls. 
It is well recognized from the community that privacy regulation in the form of differential privacy causes utility degradation on the downstream tasl including classification \cite{}, xxx \cite{}, xxx \cite{}. 
On contrary, privacy deregulation means we gradually lower the differential privacy requirement on the synthetic dataset. 
Intuitively, deregulation on the privacy requirement on tabular dataset synthesis should brings utility recovery in terms of downstream task. \textit{Well. Really?}

\textit{Para01:}
Tabular data synthesis is xxx.
(1) ...
(2) ...
(3) ... 
Under privacy regulation \cite{}, it is well-recognized by the research community that the utility degration is unaboiable. 






Such utility-privacy tradeoff is somewhat timdaing and discourage machine learning practioners. 
(1) ...
(2) ...
(3) ...
Indeed, we ask the following practical questions: Does every family generative models is capable to recover their utility under privacy deregulation? 

Unfortunately, we observed in our experiment that the DP-CTGAN methods suffers utility recovery incapability when loosen the differential privacy requirement (deregulation). That is, The relation between utility decay and differential privacy degree is observed as independent. However, we still observed PrivBayes and PATE-GAN methods enjoys utility recovery capability, and PrivBayes recovers faster than PATE-GAN. 

%\subsection
\textit{A Tale of Three Cities of Differential Privacy}
DP-CTGAN, PATE-CTGAN, PrivBayes all have their own way to ensure differential privacy.

\textit{(a)How DP-CTGAN get differential privacy?} 
Direct inject noise on SGD. DP on training.

\textit{(b)How PATE-CTGAN get differential privacy?} 
Teacher framework. DP on voting procedure. 

\textit{(c)How PrivBayes get differential privacy?}
Inject noise on the marginal noise. DP on marginal distirbution.

%\subsection
\textit{Pitfall: Utility Recovery Incapability of Neural Net-based Generative Models}

Figure \ref{fig:UtiRecoIncap} gives an example of the observed Utility Recovery Incapability of Neaural Net-based Generative Models in the task of synthetic training of classifier. 

\textit{Privacy Deregulation.}






\clearpage
---

\textbf{Tabular Data Synthesis General Overview.}


\cite{jordon2022synthetic} gives synthetic data why what how. 


\cite{cummings2018role} gives DP in GDPR.
\textbf{Degree of deregulation.}



\textbf{Differential Private Bayesian Network-based Tabular Data Generative Models.}

\textit{PrivBayes.}
Original PrivBayes network \cite{PrivBayes}.

a Naive Bayes model synthesizer with binary features\cite{avino2018generating}

PrivTree\cite{PrivTree}

Graphical-model based method private-pgm\cite{pgm}

PrivMRF (Markov random field) \cite{privmrf}

APPROX-PRIVATE-PGM (APPGM)\cite{appgm}

\textcolor{red}{What is the option to enable DP in BN-based tabular data?}





\textbf{Differential Private  Neural Network-based Tabular Data Generative Models.}


\textcolor{red}{What is the option to enable DP in NN-based tabular data?}


\textit{PATE-CTGAN.} \textcolor{red}{Make 5 works about PATE-GAN based tabular data synthesis.}

PATE framework \cite{pate}


pategan \cite{pategan}, pate-ctgan \cite{patectgan},
privacy-preserving data Generative model based on the PATE framework (G-PATE)\cite{gpate}

\textit{DP-CTGAN}

tabular gan work: Table-GAN\cite{tablegan}, TGAN \cite{tgan}, CTGAN\cite{ctgan}, CTAB-GAN \cite{ctabgan}.

Original DP algorithm \cite{DP}

GAN with DP: DPGAN\cite{dpgan}, DP-CGAN\cite{dpcgan}. \cite{frigerio2019differentially} this work does not have a name, they describe themselves as an extension to the previous dp-GAN. 
differentially private autoencoder-based generative model (DP-AuGM) and differentially private variational autoencoder-based generative model (DP-VaeGM) \cite{chen2018differentially}

Other methods:
GS-WGAN\cite{gswgan} use gradient sanitization and Wassertein distance. DP-MERF\cite{dpmerf} and PEARL\cite{pearl} use differentially private embedding. auto-encoder technique (DP-SYN)\cite{dpsyn}

Previous experiment works:
\cite{utility} our main reference. \cite{dp&pate} compare DP-SGD and PATE.
\cite{benchmarking} runs a benchmark for existing methods.



Works Compared with real dataset:  GSWGAN\cite{gswgan}, PATE-CTGAN\cite{patectgan} ( actually this is a experiment work compared many methods), DP-AuGM and DP-VaeGM proposed in the same paper \cite{chen2018differentially}.
PATE-GAN\cite{pategan} compare AUROC and AUPRC among GAN, PATEGAN and DPGAN.
DPCGAN\cite{dpcgan} compared with real dataset on LR and MLP with $\epsilon = 9.6$.



Works compared different $\epsilon$: PATE-CTGAN\cite{patectgan}. 
DP-GAN\cite{dpgan} compared Wasserstein distance for different $\epsilon = 9.6, 14, 29$. 

\cite{cummings2018role} do The role of differential privacy in gdpr compliance. 




\clearpage
---

\subsection{Differential Private Training Data Synthesis.}

%\textcolor{red}{Introduce the 4 datasets here...} 
\textbf{Source Dataset.} Our experiments are based on four commonly used machine learning datasets from UCI machine learning repository\footnote{ http://archive.ics.uci.edu/ml} and Kaggle\footnote{https://www.kaggle.com/} (see Table~\ref{datasets}). 
\textit{(i) Banknote.} The Banknote Authentication dataset involves predicting whether a given banknote is authentic given a number of measures taken from a photograph. 
\textit{(ii) Iris.} The Iris Dataset contains four features of 50 samples of three species of Iris. 
\textit{(iii) Social Network Aid.} The Social Network Ads is a categorical dataset to determine whether a user purchased a particular product. 
\textit{(iv)Banknote.} The Titanic dataset tells whether a passenger survived the sinking of the Titanic.

%\textbf{Differential Privacy.} \textcolor{red}{Give formal comparison between 3 styles of adding DP guarantee.}

\begin{table}
  \caption{Datasets}
  \label{datasets}
  \centering
  \begin{tabular}{lll}
    \toprule
    Name     & Instances     & Classes \\
    \midrule
    Banknote Authentication & 1372 & 2     \\
    Iris    & 150 & 3     \\
    Social Network Ads  & 400 & 2  \\
    Titanic & 1309 & 2  \\
    \bottomrule
  \end{tabular}
\end{table}


%\textcolor{red}{Describe how to synthesize tabular training dataset here...} 

\textbf{Tabular Training Dataset Synthesis.}  We use three methods to generate synthetic dataset with privacy-preservation. Datasynthesizer \cite{Datasynthesizer} is a Bayesian networks tool that takes a sensitive dataset as input and generates a structurally and statistically similar synthetic dataset with strong privacy guarantees. DP-CTGAN \cite{dpctgan} is a Generative Adversarial Networks (GANs), which incorporates differential privacy into a conditional tabular generative model. PATE-CTGAN \cite{patectgan} is a modified conditional tabular generative model with Private Aggregation of Teacher Ensembles (PATE) framework. These GANs based methods are implemented with open-source library of SmartNoise\footnote{https://github.com/opendp/smartnoise-sdk}. 

\subsection{Training Classifier with Synthetic Dataset.}

%\textcolor{red}{Introduce the 6 ML Classifier here.}

\textbf{Model class of Classifier.}
We approach the classification tasks by applying six different machine learning algorithms, namely Na\"ive Bayes, Support Vector Machines, K-Nearest Neighbours, Decision Tree, Random Forests and Logistic Regression. All classifiers are implemented with sklearn package\footnote{https://scikit-learn.org/stable/index.html}, and we use standard parameters.

\textbf{Synthetic Data Training Procedure.}
\textcolor{red}{Describe how we train ML classifier based on synthetic dataset.}

We train our classifier with following steps:
\begin{enumerate}
    \item Clean the original dataset by deleting some columns like names.
    \item Randomly generate ten different splits of the dateset into training data and test data, such that the size of the former is $80\%$ of the original data.
    \item For original training data and test data, apply a pre-processing procedure with label-encoding and standardization.
    \item Generate synthetic training data of same size with different $\epsilon$.
    \item Train each classifier with synthetic training data and test on original test data.
    \item Repeat Step 3-5 for each split.
\end{enumerate}

\subsection{Choice of Classification Specific Utility Metric}

\textbf{Utility metrics for classification}
\textcolor{red}{Describe 6 metrics here.}

We use 6 different metrics in our experiments, including Accuracy, Precision, Recall, F1 Score, Area Under the Receiver Operating Characteristic Curve(AUROC) and Average Precision. All metrics are implemented with sklearn package. We calculate the mean, maximum and minimum of each metric for totally 10 data splits.




\clearpage
---

How to present? Datasetwise?

Give:Dataset dimension, characteristic.
MAtch: utility recovery capability.

We test with different $\epsilon$, evenly spaced from 0 to 4, with 0.1 as the interval. We draw mean line and fill the region from the maximum to the minimum. Note that when $\epsilon=0$, Data Synthesizer is a non-privacy-preservation method. We also draw the result of original training data with a dotted line.

Due to the limited space, we only discuss the result on Banknote dataset in details and introduce briefly the difference between other datasets.

\subsection{Generative Model Utility Recovery Capability on \textit{Banknote Authentication}}
\textbf{Mean. Robustness.}



Figure \ref{banknote accuracy} shows the test accuracy of six machine learning classifier with training data which synthesized by three methods. 

First, accuracy of DP-CTGAN is always around $50\%$ no matter which classifier is used and no matter which $\epsilon$. This implies training with DP-CTGAN synthesized data is just a random guess. DP-CTGAN is not a proper method to synthesize data.

Second, the test accuracy with PATE-CTGAN starts to recover when $\epsilon > 3$. And the interval between maximum and minimum tends to shrink, which means the test accuracy with PATE-CTGAN becomes stable when $\epsilon$ increases. We can interpret this as robustness under synthesizing. This is the phenomenon shows utility recovery under PATE-CTGAN. Thus, PATE-CTGAN is a good choice when $\epsilon$ is not too small.

Finally, DataSynthesizer show best performance out of these three synthesizing methods. It has best accuracy, smallest extremum range and also a utility recovery phenomenon. This Bayesian Network method also achieve acceptable preformance when $\epsilon$ is small, which implies it is a indeed a stable method.

For other metrics, they all shows similar phenomenon as Accuracy except for Recall. Next, we only focus on Recall. Other metrics results are presented in appendix, see Appendix \ref{appendix:banknote}. 

Figure \ref{banknote recall} shows the result of Recall on Banknote dataset. On one hand, only PATE-CTGAN shows utility recovery on Recall while other two methods don't have such recovery. Datasynthesizer maintains a good recall value for most classifier. To be exact, it achieves Recall Score more than 0.6 for most cases. On the other hand, DataSynthesizer still has the smallest range from minimum value to maximum. DP-CTGAN has Recall value from 0 to 1 for most $\epsilon$. This implies DataSynthesizer is still robust on Recall metric and DP-CTGAN fails. 



\subsection{Different Results on Other Datasets}
Here we introduce the main different results found on other datasets. For detailed results and figures, see Appendix \ref{appendix:iris}, \ref{appendix:social} and \ref{appendix:titanic}.

The main difference on Iris is that PATE-CTGAN will exceed DataSynthesizer eventually when $\epsilon$ increases. When $\epsilon$ is large enough, PATE-CTGAN is a better choice compared DataSynthesizer. While DataSynthesizer has obvious advantages with small $\epsilon$.

For Social Network Ads and Titanic, PATE-CTGAN fails on utility recovery, same as DP-CTGAN. DataSynthesizer is the only method shows good performance and upward trend under $\epsilon$. Thus, DataSynthersizer is the most stable methods among these three when datasets varies. PATE-CTGAN is strongly affected by datasets and DP-CTGAN fails for all datasets we test.

%\subsection{Generative Model Utility Recovery Capability on \textit{Iris}}


%\subsection{Generative Model Utility Recovery Capability on \textit{Social Network Ads}}


%\subsection{Generative Model Utility Recovery Capability on \textit{Titanic}}


